Pragmatist: Multiview Conditional Diffusion Models for High-Fidelity 3D Reconstruction from Unposed Sparse Views

Inferring 3D structures from sparse, unposed observations is challenging due to its unconstrained nature. Recent methods propose to predict implicit representations directly from unposed inputs in a data-driven manner, achieving promising results. However, these methods do not utilize geometric priors and cannot hallucinate the appearance of unseen regions, thus making it challenging to reconstruct fine geometric and textural details. To tackle this challenge, our key idea is to reformulate this ill-posed problem as conditional novel view synthesis, aiming to generate complete observations from limited input views to facilitate reconstruction. With complete observations, the poses of the input views can be easily recovered and further used to optimize the reconstructed object. To this end, we propose a novel pipeline Pragmatist. First, we generate a complete observation of the object via a multiview conditional diffusion model. Then, we use a feed-forward large reconstruction model to obtain the reconstructed mesh. To further improve the reconstruction quality, we recover the poses of input views by inverting the obtained 3D representations and further optimize the texture using detailed input views. Unlike previous approaches, our pipeline improves reconstruction by efficiently leveraging unposed inputs and generative priors, circumventing the direct resolution of highly ill-posed problems. Extensive experiments show that our approach achieves promising performance in several benchmarks.

==> figure/ablation.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.42\textwidth]{figure/media/ablation.pdf}
    \vspace{-2mm}
    \caption{\textbf{Ablation Study on Generative Priors.} As shown above, incorporating generative priors enables the synthesis of plausible textures in unseen regions of objects.}
    \label{fig:ablation_generative}
    \vspace{-2mm}
\end{figure}

==> section/checklist.tex <==
\textbf{Reproducibility Checklist}

% list 1
\noindent 1. This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (\textcolor{blue}{Yes})
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\textcolor{blue}{Yes})
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\textcolor{blue}{Yes})
\end{itemize}

% list 2
\noindent 2. Does this paper make theoretical contributions? (\textcolor{gray}{No})
% If yes, please complete the list below.

% All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
% All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
% Proofs of all novel claims are included. (yes/partial/no)
% Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
% Appropriate citations to theoretical tools used are given. (yes/partial/no)
% All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
% All experimental code used to eliminate or disprove claims is included. (yes/no/NA)

% list 3
\noindent 3. Does this paper rely on one or more datasets? (\textcolor{blue}{Yes})
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (\textcolor{blue}{Yes})
    \item All novel datasets introduced in this paper are included in a data appendix. (\textcolor{blue}{Yes})
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textcolor{blue}{Yes})
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\textcolor{blue}{Yes})
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\textcolor{blue}{Yes})
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (\textcolor{blue}{Yes})
\end{itemize}

% list 4
\noindent 4. Does this paper include computational experiments? (\textcolor{blue}{Yes})
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (\textcolor{blue}{Yes})
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (\textcolor{gray}{Partial})
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textcolor{blue}{Yes})
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\textcolor{blue}{Yes})
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (\textcolor{blue}{Yes})
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\textcolor{blue}{Yes})
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\textcolor{blue}{Yes})
    \item This paper states the number of algorithm runs used to compute each reported result. (\textcolor{blue}{Yes})
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\textcolor{blue}{Yes})
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (\textcolor{blue}{Yes})
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\textcolor{gray}{Partial})
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\textcolor{blue}{Yes})
\end{itemize}
